GoodSpeed: Optimizing Fair Goodput with Adaptive Speculative Decoding in Distributed Edge Inference

Large language models (LLMs) have revolutionized natural language processing, yet their high computational demands pose significant challenges for real-time inference, especially in multi-user server speculative decoding and resource-constrained environments. Speculative decoding has emerged as a promising technique to accelerate LLM inference by using lightweight draft models to generate candidate tokens, which are subsequently verified by a larger, more accurate model. However, ensuring both high goodput (the effective rate of accepted tokens) and fairness across multiple draft servers cooperating with a central verification server remains an open challenge. This paper introduces GOODSPEED, a novel distributed inference framework that optimizes goodput through adaptive speculative decoding. GOODSPEED employs a central verification server that coordinates a set of heterogeneous draft servers, each running a small language model to generate speculative tokens. To manage resource allocation effectively, GOODSPEED incorporates a gradient scheduling algorithm that dynamically assigns token verification tasks, maximizing a logarithmic utility function to ensure proportional fairness across servers. By processing speculative outputs from all draft servers in parallel, the framework enables efficient collaboration between the verification server and distributed draft generators, streamlining both latency and throughput. Through rigorous fluid sample path analysis, we show that GOODSPEED converges to the optimal goodput allocation in steady-state conditions and maintains near-optimal performance with provably bounded error under dynamic workloads. These results demonstrate that GOODSPEED provides a scalable, fair and efficient solution for multi-server speculative decoding in distributed LLM inference systems.

==> Section/problem_formulation.tex <==
\section{Problem Description and Background}
\subsection{System Model}
\begin{figure}[t]
	\centering    
	\includegraphics[width=0.9\columnwidth]{Figure/System_Visualization_2.pdf}
	\caption{The visualization of the Federated PCA-based anomaly detection system model.}
	\label{fig:system}
\end{figure}
% \comment{
% As shown in Fig~\ref{fig:system}, we consider an IDS comprising a set of local security gateways (i.e. FL clients), each of which collects locally-observed traffic records from connected local IoT devices to train local models for anomaly detection. In a federated setting as previous works~\cite{Nguyen2019, Wang2022}, the local security gateways are connected to a global coordinator (i.e. FL server), which aims to continuously aggregates the local models from local gateways into a global model to cope with the privacy concerns and computational limitation of IoT devices (details in Sec.~\ref{Sec:FedPCA}). Although our methodology is generally applicable, in this paper we focus on the particular application of IDS anomaly detection. An anomaly refers to unusual traffic records in a network that are caused by service attacks.}
As shown in Fig~\ref{fig:system}, we consider a federated IDS for IoT networks. Typically, IoT systems contain multiple local gateways which each operates and monitors network traffic on a group of IoT devices. By integrating the FL processes into the gateways, we make them become security components (i.e. FL clients) performing the model training tasks on their local traffic. Those local security gateways, once deployed, will communicate with a global coordinator (i.e, FL server), which can be a cloud server, to achieve anomaly detection in a heterogeneous system. The advantage of federated IDS will not only help protect networks from malicious activities but also preserve data privacy, alleviate the computational burden of centralized approaches, improve bandwidth utilization, and further deal better with a surge of diverse data communications~\cite{Nguyen2019,Wang2022}.

The FL process between local security gateways ($GW$) and the global coordinator ($CO$) can be explained as follows. In the training phase, $CO$ and $GW$ will involve in a server-client computation to obtain the low-rank PCA representation of network traffic. Particularly, at each communication iteration, $CO$ broadcasts the current global model to $GW$s. After that, $GW$s update local models using their local data; $CO$ then aggregates the latest local models from a subset of sampled clients to update a new global model, and iterated until convergence. Once the training process is finished, $GW$s will leverage the final global model to perform PCA-based anomaly detection tasks in an unsupervised manner. We show in Sec.~\ref{Sec:FedPCA} that by using unlabelled data to train the model in a distributed setting, our proposed approach can help efficiently identify both known and unknown intrusions which are more generalizable than supervised learning approaches. Moreover, the proposed federated IDS system based on PCA is fast and lightweight (details in Sec.~\ref{Sec:FedPCA}) harmonizing with the limited-resource computing IoT devices.

\subsection{PCA for Centralized dataset}\label{Sec:CentralizedPCA}
Here, we introduce the PCA approach~\cite{Pearson1901} for centralized anomaly detection within the above system model. Assuming that each local gateway collects data, and sends the collected data to the global server, we use $X \in \mathbb{R}^{d \times D}$ to denote the fully observed dataset, where $d$ is data dimension and $D$ is the total number of data points. The dataset $X=[X_{1},X_{2}, \ldots, X_{N}]$ is distributed to $N$ clients. Each client $i \in \set{1,\ldots,N}$ contains a local dataset of $D_i$ records denoted by  $X_i = [x_{1},x_{2}, \ldots, x_{D_i}] \in \mathbb{R}^{d \times D_i}$, where $x_1\in \mathbb{R}^{d}$ represents a  record and $\SumNoLim{i=1}{N}D_i = D$.
% \begin{align*}
% 	X =
% 	\begin{bmatrix}
% 		X_{1} & X_{2} & \ldots & X_{N}
% 	\end{bmatrix}
% \end{align*}
Formally, PCA projects a given set of data onto principal components ordered by the amount of data variance that they capture~\cite{Jolliffe2002}. The PCA problem seeks the best rank-$k$ ($k < d$) matrix $\tilde{X}$ such that the reconstruction error, measured by $\norm{X - \tilde{X}}_F$, is minimized where $||\cdot||_F$ denotes the Frobenius norm~\cite{Udell2016}. Typically, the solution $\tilde{X}$ is based on the singular value decomposition of $X$, i.e.,
% \begin{align*}
	$X = U \Sigma V^\top$,
% \end{align*}
where $U \in \mathbb{R}^{d \times d}$ contains the left singular vectors of $X$ on its columns, $\Sigma = \text{diag}(\sigma_1, \ldots, \sigma_d)$ contains the singular values ($\sigma_1 \geq \sigma_2 \geq \ldots \geq \sigma_d$), and $V \in \mathbb{R}^{D \times D}$ contains the right singular vectors of $X$ on its columns. Note that the columns of $U$ are orthonormal. Let $U_k \in \mathbb{R}^{d \times k}$ be the first $k$ columns of $U$ and $\Sigma_k = \text{diag}(\sigma_1, \ldots, \sigma_k)$. We can rewrite the closed-form solution for $\tilde{X}$ as
\begin{align} \label{E:pca_centralized}
	\tilde{X} = U_k U_k^\top X,
\end{align}
which can be interpreted as the projection of data matrix $X$ onto the column space of $U_k$. 
The PCA problem can then be represented as the following optimization problem:
\begin{equation} \label{Prob:pca_centralized}
	\begin{aligned}
		\min_{U \in \mathbb{R}^{d \times k}} \quad & \norm{(I - U U^\top)X}_F^2 \\
		\mathrm{s.t.} \quad & U^\top U = I.
	\end{aligned}
\end{equation}
The above problem aims to find an orthogonal matrix $U$, captured by its constraint, such that $UU^\top X$ is the best rank-$k$ approximation of $X$.

\subsection{PCA for Network Anomaly Detection}\label{Sec:PCA-for-AD}
As discussed above, PCA aims to minimize the reconstruction error, i.e. $\norm{X - \tilde{X}}_F$, to capture the most salient information of the original features in such a way that they can reconstruct the original feature set from the reduced feature set. Given an observed record $x\in \mathbb{R}^{d}$, its reconstruction error is denoted as $||x - U_k U_k^\top x||_F^2$. Considering the fact that anomaly is rare and presumably different than normal behaviors~\cite{Patel2019}, the gist of PCA-based anomaly detection is that the anomalous records should exhibit a larger reconstruction error. In practice, we use PCA to learn a profile that represents normal behavior. As in previous works~\cite{Brauckhoff2009}, an anomaly is flagged when the reconstruction error surpasses a security threshold.  

\section{Federated PCA for Network Anomaly Detection}\label{Sec:FedPCA}
\subsection{PCA for distributed dataset}
In the previous, we see that finding $U_k$ allows us to reduce the dimension of the dataset. The quantity $Z_k = U_k^\top X \in \mathbb{R}^{k \times D}$ in \eqref{E:pca_centralized} is the lower-dimensional version of $X$ such that the reconstruction error is minimum. In the distributed setting, we aim to learn a \emph{common representation} among all client's dataset. In other words, we aim to find the rank-$k$ matrix $U$ such that the reconstruction error, averaged over all clients, is minimized. Inspired by the finite-sum formulation, we introduce the federated PCA Problem as:
\begin{equation} \label{Prob:pca_decentralized}
	\begin{aligned}
		\min_{U \in \mathbb{R}^{d \times k}} \quad & \SumLim{i=1}{N} \BigC{f_i(U) := \norm{(I - U U^\top)X_i}_F^2} \\
		\mathrm{s.t.} \quad & U^\top U = I. 
	\end{aligned}
\end{equation}
%where $f_i(U) = \norm{(I - U U^\top)X_i}_F^2$.

% \subsection{Result review}
% ADMM allows solving large-scale convex optimisation problem in a distributed manner by transferring constraint optimisation problem into sub-problems.The standard problem setting of ADMM is 
% \begin{equation} \label{Prob: ADMM}
% 	\begin{aligned}
% 		\min_{x,z} \quad & f(x) +  g(z)  \\
% 		\mathrm{s.t.} \quad & Ax + Bz - c = 0,
% 	\end{aligned}
% \end{equation}
% with variable $x\in R^n$, $z \in R^m$ and convex function $f$ and $g$, where $A \in R^{p \times n}$ and $B \in R^{p \times m}$.
% The augmented Lagrangian is
% \begin{align*}
% \mathcal{L}_\rho(x, z, y) & =  f(x) + g(z) + y^\top (Ax + Bz - c) + \frac{\rho}{2} \norm{Ax + Bz -c}^2 \\
% &= f(x) + g(z) + \frac{\rho}{2} \norm{Ax + Bz - c + u}^2 + \text{constant}
% \end{align*}
% with $u^K = (\frac{1}{\rho})y^k$. 

% Define the dual function as
% \begin{align*}
% 	d(y) = \inf_{x, z} \mathcal{L}_\rho(x, z, y).
% \end{align*}
% Then the dual problem is
% \begin{equation*} \label{Prob: ADMM_dual}
% 	\begin{aligned}
% 		\max_{y} \bigC{d(y) = \inf_{x, z} \mathcal{L}_\rho(x, z, y)}.
% 	\end{aligned}
% \end{equation*}
% ADMM iteratively updates $x$, $z$ and $u$ in each iteration $k$ as follows
% \begin{align*}
% 	x^{k+1} &= \argmin_{x} \BigC{f(x) + \frac{\rho}{2} \norm{Ax + Bz^k - c + u^k}}\\
% 	z^{k+1} &= \argmin_{z} \BigC{g(z) + \frac{\rho}{2} \norm{Ax^{k+1} + Bz - c + u^k}}\\
% 	u^{k+1} &= u^k + \rho \bigP{Ax^{k+1} + Bz^{k+1} - c}.
% \end{align*}
% Once $u^*$ is found, we can find $y^*$. Then, $x^*$ and $z^*$ can be recovered from $\mathcal{L}_\rho(x, z, y^*)$ by finding a saddle point $(x^*, z^*, y^*)$.

% \subsection{ADMM for solving consensus optimization}

% Suppose that $f$ is decomposable into $N$ functions such that $f(x) = \SumNoLim{i=1}{N} f_i(x)$. In distributed optimization, each $f_i$ can be thought of as a local objective function that is only available on device $i$. The following problem
% \begin{equation*}
% 	\begin{aligned}
% 		\min_{x_1,\ldots,x_N} \bigC{f(x) = \SumNoLim{i=1}{N} f_i(x)}
% 	\end{aligned}
% \end{equation*}
% has its ADMM equivalent as follows
% \begin{equation*}
% 	\begin{aligned}
% 		\min_{x} \quad& f(x) = \SumNoLim{i=1}{N} f_i(x_i)\\
% 		\mathrm{s.t.} \quad& x_i = z, \forall i=1,\ldots,N.
% 	\end{aligned}
% \end{equation*}
% The problem is called ``consensus'' because all local parameters must be equal (to $z$). The augmented Lagrangian is
% \begin{align*}
% 	\mathcal{L}(x, z, y) = \SumLim{i=1}{N} f_i(x_i) + \SumLim{i=1}{N} y_i^\top (x_i - z) + \frac{\rho}{2} \SumLim{i=1}{N} \norm{x_i - z}^2.
% \end{align*}
% Using the same analysis as above, we arrive at the following update rules for $x$, $z$ and $y$:
% \begin{align*}
% 	x_i^{k+1} &= \argmin_{x_i} \BigC{f_i(x_i) + y_i^{k\top}(x_i - z^k) + \frac{\rho}{2} \norm{x_i - z^k}^2} \\
% 	z^{k+1} &= \frac{1}{N} \SumLim{i=1}{N} \bigP{x_i^{k+1} + \frac{1}{\rho}y_i^k} \\ 
% 	y_i^{k+1} &= y_i^k + \rho \bigP{x_i^{k+1} - z^{k+1}}.
% \end{align*}

\subsection{ADMM for Federated PCA optimization}~\label{Sec:FedPE}
% {\small 
\begin{algorithm}[t]
	\caption{Federated PCA on Euclidean space (FedPE)}
	\label{algo1}
	\begin{algorithmic}[1]
% 		\State \tbf{Input:} $U$
		\State Randomly initialize $Z^0$ and $U_i^0, \forall i.$
		\For{$k = 0, \ldots, T - 1$} \Comment{\textit{Global rounds}}
		%\State Broadcast $Z^{k}$ to all clients
		\For {client $i = 1, \ldots, N$ in parallel} \Comment{\textit{Local rounds}} 
%  		\State $U^k_i = Z^k$
% 		\State Update $U_i$ 
% 		\begin{align*}
% 			U_i^{k+1}= &\argmin_{U_i} \BigC{f_i(U_i) + \innProd{Y_i^k, U_i - Z^k}_F \\ &+ \innProd{T_i^k, h_i(U_i)}_F + \frac{\rho}{2} \norm{U_i - Z^k}_F^2 + \frac{\rho}{2} \norm{h_i(U_i)}_F^2}
% 		\end{align*}
		\State $U_i^{k+1} = \underset{U_i}{\operatorname{\argmin}}  \BigC{f_i(U_i) + \innProd{Y_i^k, U_i - Z^k}_F + \innProd{T_i^k, h_i(U_i)}_F + \frac{\rho}{2} \norm{U_i - Z^k}_F^2 + \frac{\rho}{2} \norm{h_i(U_i)}_F^2}$
		\EndFor
% 		\State Aggregate all $U_i^{k+1}$ from clients
		\State  $CO$ updates $Z^{k+1} = \frac{1}{N} \SumNoLim{i=1}{N} U_i^{k+1}$  \Comment{\textit{Global update}}
		\State $CO$ broadcasts $Z^{k+1}$ to all clients
		\For {client $i = 1, \ldots, N$ in parallel} \Comment{\textit{Local update}}
		\State   $Y_i^{k+1} = Y_i^k + \rho \BigP{U_i^{k+1} - Z^{k+1}} $ %\Comment{Local update}
		\State   $T_i^{k+1} = T_i^k + \rho \, h_i(U_i^{k+1})$ %\Comment{Local update}
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}
% }
As discussed in Sec.~\ref{Sec:CentralizedPCA}, the centralized PCA achieves incorporation of local gateway for anomaly detection by sending their local data to a global server. However, within an IDS development, it is impractical to share local data with the server for communication costs and privacy concerns.
% \textcolor{red}{
To address the problem~(\ref{Prob:pca_decentralized}) in a privacy-preserving manner, we proposed an algorithm on Euclidean space, namely Federated PCA on Euclidean space (FedPE). In order to design FedPE following an FL style, we need to transform \eqref{Prob:pca_decentralized} into a problem that enables distributed algorithm structure. 

% }

By first introducing a set of local variables $U_1, \ldots, U_N$,  we have an equivalent problem to  \eqref{Prob:pca_decentralized} as follows:
\begin{equation} \label{Prob:pca_decentralized_admm}
	\begin{aligned}
		\min_{U_1, \ldots, U_N} \quad & { \SumLim{i=1}{N} \norm{(I - U_i U_i^\top)X_i}_F^2} \\
		\mathrm{s.t.} \quad & U_i = Z, \; \forall i=1,\ldots,N. \\
		 \quad & U_i^\top U_i = I, \; \forall i=1,\ldots,N, 
	\end{aligned}
\end{equation}
where the first linear constraint enforces the ``consensus'' \cite{Boyd2011} for all local $U_i$. The second constraint, however, is not linear in $U_i$. Using the technique in \cite{giesen2016distributed} to handle non-linear constraints in ADMM, we next define the following function 
\begin{align*}
	h_i (U_i) = \max{\set{0, U_i^\top U_i - I}}^2,
\end{align*}
where the operators $\max$ and squared are component-wise. Then, we have the problem \eqref{Prob:pca_decentralized_admm} equivalent to the following
\begin{equation} \label{Prob:pca_decentralized_admm_nonlinear}
	\begin{aligned}
		\min_{U_1, \ldots, U_N} \quad & { \SumLim{i=1}{N} \norm{(I - U_i U_i^\top)X_i}_F^2} \\
		\mathrm{s.t.} \quad & U_i = Z, \; \forall i=1,\ldots,N \\
		 \quad & h_i(U_i) = 0, \; \forall i=1,\ldots,N.
	\end{aligned}
\end{equation}
The augmented Lagrangian function associated with~(\ref{Prob:pca_decentralized_admm_nonlinear}) is
\begin{align*}
	\mathcal{L}_{\rho}(U, Z, Y, T) &= \SumLim{i=1}{N} f_i(U_i) \\
	& + \SumLim{i=1}{N}\innProd{Y_i, U_i - Z}_F + \SumLim{i=1}{N}\innProd{T_i, h_i(U_i)}_F  \\
	& + \frac{\rho}{2} \SumLim{i=1}{N} \norm{U_i - Z}_F^2 + \frac{\rho}{2} \SumLim{i=1}{N} \norm{h_i(U_i)}_F^2,
\end{align*}
where $\innProd{\cdot, \cdot}_F$ is the Frobenius inner product between two same-sized matrices where $\innProd{A, B}_F = \sum_{i, j} A_{i, j} B_{i, j} ~\text{and $A$ and $B$ are real matrices}$.

The gradient of the augmented Lagrangian with respect to dual variables $Y_i$ and $T_i$ are $\nabla_{Y_i} \mathcal{L}_{\rho}(U, Z, Y, T) = U_i - Z$ and $\nabla_{T_i} \mathcal{L}_{\rho}(U, Z, Y, T) = h_i(U_i)$.
% \begin{align*}
% 	\nabla_{Y_i} \mathcal{L}_{\rho}(U, Z, Y, T) &= U_i - Z \\
% 	\nabla_{T_i} \mathcal{L}_{\rho}(U, Z, Y, T) &= h_i(U_i).
% \end{align*}
Therefore, the ADMM updates with step side $\rho$ in each iteration $k$ \cite{Boyd2011} are
\begin{align}
	U_i^{k+1} &= \argmin_{U_i} \BigC{f_i(U_i) + \innProd{Y_i^k, U_i - Z^k}_F + \innProd{T_i^k, h_i(U_i)}_F \nonumber \\ 
		& \quad \quad \quad \quad \quad  + \frac{\rho}{2} \norm{U_i - Z^k}_F^2 + \frac{\rho}{2} \norm{h_i(U_i)}_F^2} \label{ADMM_PCA_update_U_i}. \\
	Z^{k+1} &= \frac{1}{N} \SumLim{i=1}{N} \BigP{U_i^{k+1} + \frac{1}{\rho} Y_i^k} \label{ADMM_PCA_update_Z}. \\
	Y_i^{k+1} &= Y_i^k + \rho \BigP{U_i^{k+1} - Z^{k+1}} \label{ADMM_PCA_update_Y_i}. \\
	T_i^{k+1} &= T_i^k + \rho \, h_i(U_i^{k+1}). \label{ADMM_PCA_update_T_i}
\end{align}
Substituting $Z^{k+1}$ to $Y_i^{k+1}$ leads to $\frac{1}{N} \SumNoLim{i=1}{N}Y_i^{k+1}=0$, which means $Z$ update can be rewritten as \cite{Boyd2011}:
\begin{align}
    Z^{k+1} &= \frac{1}{N} \sum_{i=1}^{N} U_i^{k+1}.
\end{align}
The whole FedPE scheme is presented in Algorithm~\ref{algo1}.
% \textcolor{red}{
The convergence of ADMM-based algorithms has been well-studied in the literature. According to the analysis results in \cite{giesen2016distributed, Hong2015,Chang2016}, the proposed FedPE algorithm guarantees convergence to a set of stationary solutions.
% } 

\subsection{Grassmann Manifold}
\begin{figure}[t]
% 	\vspace{-10pt}
	\centering    
	\includegraphics[width=0.7\columnwidth]{Figure/grassmann_manifold_AB_4.pdf}
% 		\vspace{-10pt}
	\caption{Example of moving on Grassmann manifold illustrated by a sphere. Given a point $A$ on Grassmann manifold $G$ and a vector $\Delta$ on the tangent space denoted by $\mathcal{T}_{A}G$ at $A$, a point $B$ is identified by exponential mapping $\exp_A(\Delta)$.  In our context, the manifold $G$ contains all matrix $U$ satisfy the condition $U^{\top}U = I$. }
	\label{fig:gm}
\end{figure}
% \textcolor{red}{
While FedPE can efficiently solve the proposed optimization problems, we further generalize the Federated PCA on Grassmann manifold (FedPG) as a special case of FedPE for faster convergence. Specifically, the constraint introduced in~(\ref{Prob:pca_decentralized}) implies that the parameters of (\ref{ADMM_PCA_update_U_i}) can be embedded into Grassmann manifold subspace~\cite{Jiayao2018}. In the below discussion, we first introduce the notion of the Grassmann manifold and then correlates them to our proposed algorithm in Sec.~\ref{FedPG}.
% }

Given integers $n \geq k >0$, Grassmann manifold~\cite{Jiayao2018}, denoted as $G(n,k)$, is created by all $k$-dimensional subspaces of the Euclidean space $\mathbb{R}^n$, e.g., the surface of a sphere in a 3D space depicted in Fig.~\ref{fig:gm}. According to the definition of Grassmann manifold, every element in $G(n,k)$ can be identified by selecting $n \times k$ orthogonal matrix $A$ spanning the corresponding subspace.
\begin{equation}\label{eq:grass-constraint}
	{G}(n, k) = \{ \myspan(A): A \in \mathbb{R}^{n\times k}, A^\top A= I_k\}.
\end{equation}
In the Grassmann manifold, the notion of tangent space plays a key role. Given a point $A\in G(n,k)$, a tangent space at $A$ is defined as a set of vectors $\Delta$ such that $A^{\top}\Delta = 0$.  Intuitively, a tangent space is a  vector space that contains all possible directions in which one can tangentially pass through $A$.

% Grassmanian manifold~\cite{zhang2018grassmannian} refers to a space of subspaces embedded in a higher dimensional vector space. We donate Grassmanian manifold as $G(n,k)$, with the integers $n \geq k > 0$. It refers to the space formed by all $k$-dimensional linear subspaces embedded in an $n$-dimensional real or complex Euclidean space. The Grassmanian manifold can be represented as a collection of $n\times k$ orthogonal matrix $A$ whose column spans the corresponding subspace. 
% \begin{equation}\label{eq:grass-constraint}
% 	\mathbb{G}(n, k) = \{ \myspan(A): A \in \mathbb{R}^{n\times k}, A^\top A= I_k\}.
% \end{equation}
% To solve a gradient-based learning problems in Grassmanian manifold, the notion of tangent space is required. Given a point $A\in G(n,k)$, tangent space is defined as a set of vectors $\{\nabla\}$ such that $A^{\top}\nabla = 0$.  Intuitively, tangent space is a real vector space that contains the possible directions in which one can tangentially pass through $A$.
Consider a function $F: {G(n,k) \rightarrow \mathbb{R}}$ and its Euclidean gradient $F_A$ at point $A$, 
the projected gradient of the function $F$ on the Grassmann manifold is computed by projecting the Euclidean gradient $F_A$ onto the tangent space of the Grassmann manifold using the orthogonal projection $F_A \rightarrow \nabla_A{F}$:
\begin{equation}
	\nabla_AF\ = (I_k - AA^{\top})F_A.
\end{equation}
The aim is to compute a forward step in the direction of the projected gradient on the Grassman manifold. While the projection from the tangent plane to the manifold can be done by using exponential mapping, this approach is expensive in terms of computation. Alternatively, the retraction function is introduced as a local approximation of exponential mapping on the manifold with less computation complexity \cite{sato2019riemannian}. 
Thus, a retraction operation is performed by mapping the tangent matrix back on the manifold:
\begin{equation}
	B = R(A -\eta \nabla_A F),
\end{equation}
where $\eta$ is the step size and $R$ is the retraction function on the Grassmann manifold performed by applying QR decomposition \cite{Jiayao2018}. 

\subsection{Distributed PCA using ADMM and Grassmann manifold}~\label{FedPG}
\begin{algorithm}[t]
    % \algsetup{linenosize=\tiny}
    % \small
	\caption{Federated PCA on Grassmann manifold (FedPG)}
    \label{algo2}
	\begin{algorithmic}[1]
% 		\State \tbf{Input:} $U$
		\State Randomly initialize $Z^0$ and $U_i^0, \forall i$
		\For{$k = 0, \ldots, T - 1$} \Comment{\textit{Global  rounds}}
	%	\State Broadcast $Z^{k}$ to all clients

		\For {client $i = 1, \ldots, N$ in parallel} 
 		\State $U^{k, 0}_i = U^{k}_i$
% 		\tcp*[f]{Local rounds}
		\For{$c = 0, \ldots, C - 1$} \Comment{\textit{Local rounds}}
		\State $\nabla_U F_i^k(U_i^{k,c}) = (I_d - U_i^{k,c}U_i^{k,c \top}) F_i^k(U_i^{k,c})$ 
		\State $U_{i}^{k, c+1} =R(U_i^{k, c} - \eta \nabla_U F_i^k(U_i^{k,c}))$
		\EndFor
		\State $U_i^{k+1} = U_{i}^{k, C} $
		\EndFor
% 		\State Aggregate all $U_i^{k+1}$ from clients
		\State  $CO$ updates $Z^{k+1} = \frac{1}{N} \SumNoLim{i=1}{N} U_i^{k+1}$\Comment{\textit{Global update}}
		\State $CO$ broadcasts $Z^{k+1}$ to all clients %https://www.overleaf.com/project/60c1859569c4be9bf761503d
		\For {client $i = 1, \ldots, N$ in parallel} \Comment{\textit{Local update}}
		\State   $Y_i^{k+1} = Y_i^k + \rho \BigP{U_i^{k+1} - Z^{k+1}} $ %\Comment{Local computation}
		\State   $T_i^{k+1} = T_i^k + \rho \, h_i(U_i^{k+1})$ %\Comment{Local update}
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}
% \textcolor{red}{
Recapping the introduced problem~\eqref{Prob:pca_decentralized_admm_nonlinear}, we next propose an algorithm, namely Federated PCA on Grassmann manifold (FedPG), summarized in Algorithm~\ref{algo2}. Similar to the previous solution in Sec~\ref{Sec:FedPE}, we first enforce the consensus constraints through ADMM, then the augmented Lagrangian is
% }
\begin{equation}
\begin{split}
	\mathcal{L}(U, Z, Y) &= \SumLim{i=1}{N} f_i(U_i) + \SumLim{i=1}{N} Y_i^\top (U_i - Z) \\
	&+ \frac{\rho}{2} \SumLim{i=1}{N} \norm{U_i - Z}^2_F.
\end{split}
\end{equation}
We re-form the update rules for $U_i$ and $Z$ on the Grassmann manifold as follows: 
\begin{align} \label{E:Fopt}
	U_i^{k+1} &= \argmin_{U_i} \BigC{F_i^k(U_i)} \quad \mathrm{s.t.}
	%F_i^k(U_i) &:= f_i(U_i) + Y_i^{k\top}(U_i - Z^k) + \frac{\rho}{2} \norm{U_i - Z^k}^2.
% 	Z^{k+1} &= \frac{1}{N} \SumLim{i=1}{N} \bigP{U_i^{k+1} + \frac{1}{\rho}Y_i^k}. \\ 
% 	Y_i^{k+1} &= Y_i^k + \rho \bigP{U_i^{k+1} - Z^{k+1}}.
\end{align}

\begin{align} \label{E:Fopt_2}
	%U_i^{k+1} &= \argmin_{U_i} \BigC{F_i^k(U_i)} \quad \mathrm{s.t.}
	F_i^k(U_i) &:= f_i(U_i) + Y_i^{k\top}(U_i - Z^k) + \frac{\rho}{2} \norm{U_i - Z^k}_F^2.
% 	Z^{k+1} &= \frac{1}{N} \SumLim{i=1}{N} \bigP{U_i^{k+1} + \frac{1}{\rho}Y_i^k}. \\ 
% 	Y_i^{k+1} &= Y_i^k + \rho \bigP{U_i^{k+1} - Z^{k+1}}.
\end{align}
% The other constraint $U^TU = I$ is based on orthogonality. 
In Algorithm \ref{algo2}, as shown in lines 5-8, projected gradient descent on the Grassmann manifold is applied at every local iteration in client for finding the update of $U_i^{k+1}$ in \eqref{E:Fopt}. Considering the definition of the Grassmann manifold in (11), we enforce the second constraint $U_i^TU_i = I$ by using the projected gradient descent on the Grassmann manifold (line 7) as follows
\begin{align}
	U^{k+1}_i = R(U^k_i - \eta \nabla_U F_i^k(U^k_i)), \label{E:Gpro1}
\end{align}
where $\eta$ is the step size, and $\nabla_U F_i^k(U^k_i)$ is the gradient of $F_i^k(U^k_i)$ at point $U_i^k$, and the retraction function $R(\cdot)$ is the projection operation. Pictorially, $U^{k}_i$ and $U^{k+1}_i$ are illustrated by points $A$ and $B$ in Fig.~\ref{fig:gm}, respectively. We compute the updates by projecting the Euclidean gradient onto the tangent space of the manifold using orthogonal projection $F_i^k(U^k_i)\rightarrow  \nabla_U F_i^k(U^k_i)$ (line 6 ) as follows.
\begin{equation}
	\nabla_U F_i^k(U^k_i) = (I_d - U_i^{k}U_i^{k \top})F_i^k(U^k_i). \label{E:Gpro2}
\end{equation}
Note that the two equations \eqref{E:Gpro1} and \eqref{E:Gpro2} are repeatedly updated in $C$ local rounds at lines 5-8 in Algorithm~\ref{algo2} to solve the equation \eqref{E:Fopt}. 
% \blue{Make a connection to Fig. 2 by referencing point A to $U^k$ and B to $U^{k+1}$, $\Delta$ to $\nabla_U F_i^k(U^k_i)$. Draw new projection line in Fig. 2 to illustrate the retraction operation.}

The updates of $Y_i^k, T_i^k$ and $Z_i^k$ are identical to (8), (9) and (10), respectively.

%Note that the operation $R$ is a projection on the manifold, defined as $R(U_i)=\myspan(U_i)$. 

\subsection{Computational Complexity}\label{Sec:Complexity}
Here, we study the strength of computational complexity of the proposed algorithm FedPG. We recall that   $d$ and $k$ denote the input data dimension and the number of PCA components, respectively. $C$ and $T$ denote the number of local and global rounds, respectively.

In FedPG, the major local-client computational costs in each global communication round come from two parts, calculating the gradient updates for the matrix $U_i^k$ (Lines 7-8 in Algorithm~\ref{algo2}) and performing consensus updates for the matrices $Y$ and $T$ (Lines 15-16 in Algorithm~\ref{algo2}). Especially, computing the orthogonal projection to obtain the gradient costs at most $O(2d^2k + 2dk)$ flops for two matrix-matrix multiplications (Line 7 in Algorithm~\ref{algo2}). Once the gradient is calculated, the retraction of the update step on the Grassmann manifold is done by applying QR decomposition with complexity $O(dk + dk^2)$ (Line 8 in Algorithm~\ref{algo2}). The $Y$ and $T$ update phase needs simple matrix-matrix multiplication requiring $O(d^2k)$ flops (Line 16 in Algorithm~\ref{algo2}). Suppose the algorithm is terminated after $C$ rounds, then the overall computational complexity for each local security gateway is given by $O(C(d^2k + dk + dk^2))$. Therefore, FedPG's  complexity is (i) independent of the data side $D_i$, and (ii) dominated by two factors $d$ and $k$. In IDS applications, the network data is often not too high-dimensional (i.e, the value of $d$ is not too large~\cite{Thakkar2020} and $k < d$, as confirmed in the experiments in next section) making this computational complexity acceptable for limited-resource computing IoT devices.

At each global communication round, the global coordinator mainly updates the matrix $Z$ by averaging the sum of $U$ matrices from a subset $S = |10\%N|$ client number, hence costing $O(Sdk)$ flops.  This leads to the overall computational complexity of the global coordinator for $T$  rounds as $O(TSdk)$ flops.

==> Section/problemformulation/algorithmdesign.tex <==
\subsection{Algorithm Design}
\begin{algorithm}[t]
\caption{Speculative Decoding with Multiple Draft Clients}
\label{algo:spec_decoding}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} 
\STATE \hspace{1em} Primal model: $M_p$
\STATE \hspace{1em} $n$ client models: $M_{q_1}, \ldots, M_{q_n}$
\STATE \hspace{1em} $n$ draft length $S$: $S_1, \ldots, S_n$
\STATE \hspace{1em} Prefix prompts: $\mathbf{p}_1, \ldots, \mathbf{p}_n$

\STATE Initialise $bh\_fin \leftarrow true$, $S(0), X(0)$
\vspace{0.5em}
\STATE \textbf{Step 1: Client-side Drafting}
\FOR{$i = 1$ to $n$}
    \FOR{$j = 1$ to $S_i$}
        \STATE $q_{ij}(c) \leftarrow M_{q_i}(\mathbf{p}_i + [c_{i1}, \ldots, c_{i,j-1}])$
        \STATE Sample draft token: $c_{ij} \sim q_{ij}(c)$
    \ENDFOR
\ENDFOR

\vspace{0.5em}
\STATE \textbf{Step 2: Primal Verification}
\IF{$bh\_fin$}
% \STATE // Form a batch 
\STATE $\mathcal{B} \leftarrow$ pick $b$ draft requests from FIFO queue
\STATE $bh\_fin \leftarrow false$
\ELSE
\STATE $\mathcal{B} \leftarrow \text{next iteration from previous $b$ draft requests}$
\ENDIF
% \STATE Compute primal predictions: 
\STATE $P(C) \leftarrow M_p(\mathcal{B})$
\FOR{$i = 1$ to $b$}
    % \STATE Sample uniform noise: 
    \STATE $r_1, \ldots, r_{S_i} \sim Uniform(0,1)$
    % \STATE \textbf{// Determine accepted prefix length}
    \STATE $n_i \leftarrow \min\left(\{j-1 \mid 1 \leq j \leq S_i, r_j > \frac{P[i]_j(c)}{q_{ij}(c)}\} \cup \{S_i\}\right)$
    % \vspace{0.3em}
    % \STATE \textbf{// Construct final token distribution}
    \IF{$n_i < S_i$}
        \STATE $P'[i](c) \leftarrow \text{Norm}\left(\max\left(0, P[i]_{n_i+1}(c) - q_{i,n_i+1}(c)\right)\right)$
    \ELSE
        \STATE $P'[i](c) \leftarrow P[i]_{n_i+1}(c)$
    \ENDIF
    \STATE Sample final token: $c_{i,n_i+1} \sim P'[i](c)$
\ENDFOR
\IF{All requests hit $eos\_token$}
\STATE $bh\_fin \leftarrow true$
\ENDIF
\vspace{0.5em}
\STATE \textbf{Update}
\STATE 
\begin{equation*}
    \alpha_i(t) \leftarrow (1 - \eta) \alpha_i(t-1) 
                + \eta\frac{1}{S_i(t)} \sum_{j=1}^{S_i(t)} \min\left(1, \frac{p_{i,j}(x_{i,j})}{q_i(x_{i,j})}\right)
\end{equation*}
\STATE $X(t) \leftarrow (1 - \beta) X(t-1) + \beta x_i(t)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{\textsc{Optimization for New Draft Length $S$ Proposal}}
    \label{algo:gamma_opt}
    \begin{algorithmic}[1]
    \STATE \textbf{Inputs:}
    \STATE \hspace{1em} Decision set $K^{(m)}$ based on condition $m$
    \STATE \hspace{1em} $S(t)$: Draft lengths $(S_1, \ldots, S_n)$
    \STATE \hspace{1em} $\alpha(t)$: Acceptance rates $(\alpha_1, \ldots, \alpha_n)$
    \STATE \hspace{1em} $X(t)$: Accepted tokens $(X_1, \ldots, X_n)$
    \STATE \textbf{At time $t$, find the set of scheduling decision $k(t)$:}
    \STATE $k(t) \leftarrow \arg\max_{k \in K^{(m)}} \nabla U(X(t)) \cdot \hat{x}(t+1)$
    \STATE where:
    \STATE $\hat{x}_i(t+1) = \frac{1 - \alpha_i(t)^{S_i(t+1) + 1}}{1 - \alpha_i(t)}$
    \STATE Update proposed draft lengths and send back to clients
    \end{algorithmic}
\end{algorithm}

==> experiment_setting.tex <==
\section{Description of the Dataset}

The KDDCup’99 dataset has been known as one of the most popular dataset for anomaly detection. This dataset has been developed based on the DARPA 98 dataset at the MIT Lincoln Laboratory, produced by the DARPA (1998) Intrusion Detection Evaluation Program. It included nine weeks of raw TCP dump data for a local area network (LAN) simulating a typical US Air Force LAN. The LAN was operated as if it were a true Air Force environment, but peppered with multiple attacks. Protocols such as TCP, UDP, and ICMP had been used on this dataset to evaluate the intrusion detection methods. The full KDDCup’99 dataset (uncompressed file kddcup.data.gz) has 4,898,431 records, and each record contains 41 features. Since the KDDCup’99 dataset contains so much data, many authors used a reduced version of the KDDCup’99 dataset (uncompressed file kddcup.data 10 percent.gz) to reduce the computation time. The kddcup.data 10 percent.gz is about 10\% of the KDDCup’99 dataset, and contains 494,021 records, of which 97,278 are normal (19.6\%) and 396,743 are intrusions (80.4\%). In the reduced version, the normal, neptune, smurf, ipsweep, nmap, portsweep, and satan instances are reduced. However, because even rare intrusion instances may severely compromise security, we used the full dataset for our experiments.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{sec.~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Sec.~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{secs. \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{Secs. \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{alg.~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Alg.~\ref{#1}}
\def\twoalgref#1#2{algs. \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algs. \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_content.tex <==
\section{Math Content}
To simplify notation, denote $\gF \defeq \ell \,\circ \, \gH \defeq \set{ z \mapsto \ell(z,h), h \in \gH }.$ 

We have
\begin{align}
	{\mathscr{L}(\widehat{P}_{\lambda}, f_{\theta}) :=
	\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}} \\
{\mathscr{L}({P}, f_{\theta}) \defeq \mathbf{E}_{Z \sim {P}} \bigS{\ell(Z,  h_{\theta})}}. \\
{\mathscr{L}({P}, f) \defeq \mathbf{E}_{Z \sim {P}} \bigS{\ell(Z,  h)}}.
\end{align}

\begin{align}
\mathscr{L}_{\rho}^{\gamma} (\widehat{P}_{\lambda},f) := & \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}\Big{[}\phi_\gamma(Z, h)\Big{]} + \gamma \rho \\
\mathscr{L}_{\rho}^{\gamma} ({P},f) := & \mathbf{E}_{Z \sim {P}}\Big{[}\phi_\gamma(Z, h)\Big{]} + \gamma \rho. 
\end{align}

\textbf{Raginsky}: Suppose that $f$ is $L$-Lipschitz
\begin{align}
\mathscr{L}(Q, f) &\leq \mathscr{L}_{\rho}(P_{\lambda},f) \leq \mathscr{L}(Q,f) + 2L\rho, \;\forall Q \in \gB(P_{\lambda}, \rho) \\
\mathscr{L}(Q, f) &\leq \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \leq \mathscr{L}(Q,f) + 2L\rho, \;\forall Q \in \gB(P_{\lambda}, \rho)
\end{align}


\textbf{Proposition 1}: Suppose that $f$ is $L$-Lipschitz
\begin{align}
\mathscr{L}(Q,f) &\leq   \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f) \leq  \mathscr{L}(Q,f) + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \, {\rho}, \;\forall Q \in \gB(P_{\lambda}, \rho) \\
%\mathscr{L}(Q,f) &\leq   \mathscr{L}(P_{\lambda},\phi_{\gamma}) \leq  \mathscr{L}(Q,f) + (2L + \gamma\mathbf{I}) \, {\rho}, \;\forall Q \in \gB(P_{\lambda}, \rho)
\end{align}

\begin{proof}
	The first inequality:
	\begin{align}
	\mathscr{L}(Q,f) \leq  \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f)  \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f) \\
%	\mathscr{L}(Q,f) \leq  \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \leq  \mathscr{L}(P_{\lambda},\phi_{\gamma})
	\end{align}
	
	The last "$ \leq $":
	
	\begin{align*} 
%	\mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)  & =  \mathscr{L}_{\rho}(P_{\lambda},f) + \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f)  - \mathscr{L}_{\rho}(P_{\lambda},f) \\
	\mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)   & =   \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) + \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)  - \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \\
	&\leq   \mathscr{L}(Q,f) + 2L\rho  + \mathbf{E}_{Z \sim P}[\phi_{\gamma}(Z, h)] + \rho\gamma - \min_{\gamma^{\prime} \geq 0} \Big\{ \rho \gamma^{\prime} + \mathbf{E}_{Z \sim P}[\phi_{\gamma'}(Z, h)] \Big\} \\
	& \leq   \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\bigg\{{\rho}(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\Big[\phi_{\gamma}(Z, h) - \phi_{\gamma'}(Z, h)\Big]\bigg\} \\
	& =  \begin{aligned}[t] \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\Bigg\{\rho(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\bigg[& \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h)  - \gamma d(\zeta,  Z) \Big\} \\ 
		& \quad - \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h) - \gamma^{\prime} d(\zeta,  Z)  \Big\} \bigg]\Bigg\} \end{aligned} \\
	& =  \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\Bigg\{\rho(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\bigg[\sup_{\zeta \in \mathcal{Z}} \Big\{(\gamma^{\prime} - \gamma) d(\zeta,  Z)\Big\}\bigg]\Bigg\} \\
	& =  \mathscr{L}(Q,f) + 2L\rho + \underbrace{\max_{k \leq \gamma}\Bigg\{k\bigg(\rho - \mathbf{E}_{Z \sim P}\Big[\sup_{\zeta \in \mathcal{Z}} d(\zeta,  Z)\Big]\bigg)\Bigg\}}_{A} \\
	& \leq   \mathscr{L}(Q,f) + (2L + \gamma \, \mathbbm{1}_{\{\gamma \neq \gamma^{\prime}\}})\rho
	\end{align*}
	
	where $ k = \gamma - \gamma^{\prime} \Rightarrow \gamma^{\prime} = \gamma - k \geq 0 $
	because 
	\[
	A \leq \left\{\begin{array}{cc}{\gamma}{\rho} & \text { if } \rho \geq \mathbf{E}_{Z \sim P}\Big[\underset{\zeta \in \mathcal{Z}}{\sup}\big\{d(\zeta, Z)\big\}\Big]  \Rightarrow k=\gamma \\ 
	 \\ 0 & \text { if } \rho < ... \ k=0\end{array}\right.
	\]
	
\end{proof}

\begin{lemma} Suppose that $f'$ is $L_z$-Lipschitz
	 \[
	 	 \mathscr{L}(Q, f') - \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f') - \inf_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho, \; \forall Q \in \gB(P_{\lambda}, \rho). 
	 \]
	
\end{lemma}

\begin{proof}
	From proposition 1 and when $f_Q = \argmin_{f \in \mathcal{F}} \mathscr{L}(Q, f)$ is $L$-Lipschitz, we have:
	\begin{align}
		\mathscr{L}(Q, f') &\leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f'),  \\ 
		\inf_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_Q) &\leq \mathscr{L}(Q, f_{Q}) + (2 L+\gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho \\
		&= \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) + (2 L+\gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho. 
	\end{align}
	where  

\end{proof}

%\begin{theorem} If Assumption $\ell(Z,f)$ is $L_{\theta}$-Lipschitz continuous, then 
%	\[ 
%		\mathscr{L}(P_{\lambda}, \widehat{f}_{\theta^{\sigma}})- \inf_{f \in \mathcal{F}} \mathscr{L}(P_{\lambda}, f) \leq  \frac{\mathscr{C}(\gF)}{\sqrt{n}}+\epsilon + M \sqrt{\frac{2 \log (2 / \delta)}{n}} + (2L + \gamma) \hat{\rho}
%	\]
%	where:  
%	$\mathcal{F} = \bigC{f_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$ and  $ \widehat{f}_{\theta^{\sigma}} \in \underset{\theta \in \Theta}{\operatorname{argmin}}\ \mathscr{L}(\widehat{P}_{\lambda}, f_{\theta}) + \sigma$, and 
%	$\mathscr{C}(\mathcal{F}):=\int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\mathcal{F},\|\cdot\|_{\infty}, \epsilon \right)} \mathrm{d} \epsilon$ and $\mathcal{N}\left(\mathcal{F},\|\cdot\|_{\infty}, \epsilon \right)$ denotes the covering number of $\mathcal{F}$ in the uniform metric $\ldots$.
%\end{theorem}

\begin{theorem} \label{Thrm:key} If Assumption $\ell(z,h_{\theta})$ is $L_{\theta}$-Lipschitz continuous, $\abs{\ell(z,h) } \leq M_{\ell}$ and considering the parametrized hypothesis class  $\mathcal{H} = \bigC{h_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$, and $\forall Q \in \gB(P_{\lambda}, \rho)$, then 
	\[ 
	\mathscr{L}(Q, {f}_{\widehat{\theta}^{\varepsilon}})- \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) \leq  \sum_{i=1}^{m} \lambda_i \BiggS{\frac{48 \mathscr{C}(\Theta)}{\sqrt{n_i}} + 2 M_{\ell} \sqrt{\frac{2 \log (2  m / \delta)}{n_i}}} +\varepsilon + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho
	\]
	with probability at least $1 - \delta$. Here $\widehat{\theta}^{\varepsilon}$ is the solution returned by FedRob after $O(1/\varepsilon)$ iterations, i.e., 
	  \begin{align}
	%  \mathscr{L}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) &\defeq \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\widehat{\theta}^{\varepsilon}})}  \leq \underset{\theta \in \Theta} {\operatorname{inf}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}  + \varepsilon \\
	  \mathscr{L}_{\rho}^{\gamma} (\widehat{P}_{\lambda},f_{\widehat{\theta}^{\varepsilon}})  & \defeq \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}\Big{[}\phi_\gamma(Z, h_{\widehat{\theta}^{\varepsilon}})\Big{]} + \gamma \rho \leq \underset{\theta \in \Theta} {\operatorname{inf}}  \BigS{\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}  + \gamma \rho } + \varepsilon
%	  {\widehat{\theta}^{\varepsilon}} \in \underset{\theta \in \Theta} {\operatorname{argmin}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}  + \varepsilon
	  \end{align}
	  and 
	$\mathscr{C}(\Theta):= L_{\theta} \int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\Theta,\|\cdot\|_{\Theta}, \epsilon \right)} \mathrm{d} \epsilon$ where $\mathcal{N}\left(\Theta,\|\cdot\|_{\Theta}, \epsilon \right)$ denotes the $\epsilon$-covering number of $\Theta$ w.r.t  a  metric $\|\cdot\|_{\Theta}$ as the norm on $\Theta$.
\end{theorem}

\textbf{Remarks:}
Choose $\varepsilon$ in the order of $1/\sqrt{n}$. 

\begin{proof}
	To simplify notation, we denote $ \Phi \defeq \phi_{\gamma} \circ \mathcal{H} = \set{z \mapsto \phi_{\gamma}(z, h), h \in \mathcal{H}}$ where $\mathcal{H} = \bigC{h_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$, which represents the composition of $\phi_{\gamma}$ with each of the predictor function $h_{\theta}$ parametrized by $\theta$ belonging to a parameter class $\Theta$. 
	
	Defining $f_P \in \argmin_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f)$ and $ \widehat{\theta}^* \in \underset{\theta \in \Theta} {\operatorname{argmin}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}$ such that $\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^*}) = \underset{\theta \in \Theta} {\operatorname{inf}}  \BigS{\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}  + \gamma \rho }$, we  decompose the excess risk as follows:
	
	\begin{align}
	&\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \inf_{f \in \mathcal{F}}  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) \nonumber\\
	&= \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) -   \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_P)\nonumber\\
	&=  \BigS{\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}})} + \underbrace{\BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{*}})} }_{\leq \varepsilon} + \underbrace{\BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{*}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f_P)}}_{\leq 0} \nonumber\\
	& \quad  + \BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f_P) - \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_P)} \nonumber\\
%	& \leq 2 \sup_{f \in \mathcal{F}} \; \big\lvert\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f) \big\rvert  + \varepsilon\\
	&\leq 2 \sup_{\phi_{\gamma} \in \Phi} \abs*{ \mathbf{E}_{Z \sim P_{\lambda}}[\phi_{\gamma}(Z, h_{\theta})] -   \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}[\phi_{\gamma}(Z, h_{\theta})] } + \varepsilon \nonumber\\
	&\leq 2 \sup_{\phi_{\gamma} \in \Phi}  \sum_{i=1}^{m} \lambda_i \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  + \varepsilon \nonumber\\
	&\leq 2   \sum_{i=1}^{m} \lambda_i \sup_{\phi_{\gamma} \in \Phi} \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  + \varepsilon \nonumber\\
	%&\stackrel{\text {with prob. } \geq 1-\delta}{\leq}  
	& \leq  \sum_{i=1}^{m} \lambda_i  \biggS{4 \mathscr{R}_{i}(\Phi)+  2 M_{\ell} \sqrt{\frac{2 \log (2 m / \delta)}{n_i}}} + \varepsilon\, \text{  with probability at least }  1-\delta, \label{unionbound1}
	\end{align}
where the first inequality is due to optimization error and definition of $\widehat{\theta}^{*}$. The second inequality is due to the fact that $ \abs{\sum_{i=1}^m \lambda_i a_i } \leq \sum_{i=1}^m \lambda_i  \abs{a_i}, \forall a_i \in \mathbb{R}$ and $\lambda_i \geq 0$. The third inequality is because pushing the $\sup$ inside increases the value. For the last inequality, using  the facts that (i) $\abs{\phi_{\gamma}(z,h)} \leq M_{\ell}$  due to $-M_{\ell} \leq \ell(z, h) \leq \phi_{\gamma}(z, h) \leq \sup _{z \in \gZ} \ell(z, h) \leq M_{\ell}$ and (ii) the Rademacher complexity of the function class $\Phi$ defined by $\mathscr{R}_{i}(\Phi) = \mathbf{E}[\sup _{\phi_{\gamma} \in \Phi} \frac{1}{n_i} \sum_{k=1}^{n_i} \sigma_{k} \phi_\gamma(Z_k,  h_{\theta})] $ where the expectation is w.r.t both $Z_k \stackrel{\text { i.i.d. }}{\sim} P_i$ and i.i.d. Rademacher random variable $\sigma_{k}$ independent of $Z_k, \forall k \in [n_i]$,  we have 
\begin{align}
\sup_{\phi_{\gamma} \in \Phi} \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  \geq 2 \mathscr{R}_{i}(\Phi)+   M_{\ell} \sqrt{\frac{2 \log (2 m / \delta)}{n_i}} \label{Rade1}
\end{align}
with probability $\leq \delta/m$ due to the standard symmetrization argument and McDiarmid's inequality \blue{[UnderstandingML, Theorem26.5]}. Multiplying $\lambda_i$ to both sides of \eqref{Rade1}, summing up the inequalities over all $i\in [n]$, and using union bound, we obtain \eqref{unionbound1}.


%Conditioning on the vector $Z_1^n \defeq (Z_k)_{k\in [n]}$, the above expectation gives us the empirical Rademacher complexity denoted by $\widehat{\mathscr{R}}_{n}(\Phi)$. 
Define a stochastic process $\left(X_{\phi_{\gamma}}\right)_{\phi_{\gamma} \in \Phi}$ 
$$
X_{\phi_{\gamma}}:=\frac{1}{{\sqrt{n_i}}} \sum_{k=1}^{n_i} \sigma_{k} \phi_{\gamma}(Z_k, h_{\theta})
$$
which is  zero-mean because $\mathbf{E}\left[X_{\phi_{\gamma}}\right]=0$ for all $\phi_{\gamma} \in \Phi$.  To upper-bound  $\mathscr{R}_{n}(\Phi)$, we first show that $\left(X_{\phi_{\gamma}}\right)_{\phi_{\gamma} \in \Phi}$ is a sub-Gaussian process with respect to the following pseudometric
\begin{align}
%\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{L_2(\widehat{P}_{\lambda})}  \defeq \biggP{\frac{1}{n} \sum_{k=1}^{n}  \BigP{\phi_{\gamma}(Z_k, f_{\theta}) - \phi_{\gamma}(Z_k, h_{\theta'})}^2}^{1/2}. 
\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty}  \defeq  \sup_{z \in \mathcal{Z}} \Big\lvert  {\phi_{\gamma}(z, h_{\theta}) - \phi_{\gamma}(z, h_{\theta'})}  \Big\rvert . 
\end{align}  

For any $t \in \mathbb{R}$,  using Hoeffding inequality with the fact that $\sigma_{k}, k \in [n]$, are i.i.d. bounded random variable with sub-Gaussian  parameter 1, we have
$$
\begin{aligned}
\mathbf{E}\left[\exp \left(t\left(X_{\phi_{\gamma}}-X_{\phi_{\gamma}^{\prime}}\right)\right)\right] &=\mathbf{E}\left[\exp \left(\frac{t}{\sqrt{n_i}} \sum_{k=1}^{n_i} \sigma_{k}\left(\phi_{\gamma}\left(Z_k, h_{\theta}\right)-\phi\left(Z_k, h_{\theta'}\right)\right)\right)\right] \\
&=\left(\mathbf{E}\left[\exp \left(\frac{t}{{\sqrt{n_i}}} \sigma_{1}\left(\phi_{\gamma}\left(Z_{1}, h_{\theta}\right)-\phi_{\gamma}\left(Z_{1}, h_{\theta'}\right)\right)\right)\right]\right)^{n_i} \\
%& \leq \exp \left(\frac{t^{2} \left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{L_2(\widehat{P}_{\lambda})}^{2}}{2 }\right). 
& \leq \exp \left(\frac{t^{2} \left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty}^2}{2 }\right). 
\end{aligned}
$$
Then, invoking Dudley entropy integral, we have
\begin{align}
\sqrt{n_i}\, {\mathscr{R}}_{i}(\Phi) = \mathbf{E} \sup_{\phi_{\gamma} \in \Phi} X_{\phi_{\gamma}} \leq {12} \int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\Phi, \norm{\cdot}_{\infty}, \epsilon\right)} \mathrm{d} \epsilon
\end{align}

We will show that when $\theta \mapsto \ell(z,h_{\theta})$ is $L_{\theta}$-Lipschitz, then $\theta \mapsto \phi_{\gamma}(z, h_{\theta})$ is also $L_{\theta}$-Lipschitz. First, we have
\begin{align*}
	\Big|\phi_{\gamma}(z, h_{\theta}) - \phi_{\gamma}(z, h_{\theta'})\Big|  &=  \bigg| \sup_{\zeta \in \mathcal{Z}} \inf_{\zeta' \in \mathcal{Z}} \Big\{ \ell(\zeta,h_{\theta})  - \gamma d(\zeta,  z)   -   \ell(\zeta', h_{\theta'}) + \gamma d(\zeta',  z)  \Big\} \bigg| \\
	&\leq  \bigg| \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h_{\theta})    -   \ell(\zeta, h_{\theta'})   \Big\} \bigg| \\
	&\leq \sup_{\zeta \in \mathcal{Z}}  \bigg| \Big\{ \ell(\zeta,h_{\theta})    -   \ell(\zeta, h_{\theta'})   \Big\} \bigg| \\
	& \leq L_{\theta}   \norm{\theta - \theta'}, \\
	%& \leq L_f L_{\theta} \norm{\theta - \theta'}
\end{align*}
which implies
\begin{align}
\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty} \leq  L_{\theta}   \norm{\theta - \theta'}.
\end{align}
Therefore, by contraction principle \blue{[Understanding ML]}, we have
\begin{align}
\mathcal{N}\left(\Phi, \norm{\cdot}_{\infty}, \epsilon\right) \leq \mathcal{N}\left(\Theta, \norm{\cdot}, \epsilon/L_{\theta}\right)
\end{align}
\end{proof}

\begin{proposition}[Measure concentration (Fournier and Guillin, 2015, Theorem 2)]\label{WassRate}
	Let $P$ be a probability distribution on a bounded set $\mathcal{Z}$. Let $\widehat{P}_{n}$ denote the empirical distribution of $Z_{1}, \ldots, Z_{n} \stackrel{\text { i.i.d. }}{\sim} P.$ Assuming that there exist constants $a>1$  such that $A \defeq \mathbf{E}_{Z \sim P}\bigS{\exp(\norm{Z}^a)} < \infty$ (i.e., $P$ is a light-tail distribution). Then, for any $\rho > 0$,
$$
%\mathbf{P}\left[ W (P_{\lambda}, \widehat{P}_{n}) \geq  \rho \right] \leq c_{1} \exp \left(-c_{2} n \rho^{\max\{d+1, 2\}}\right) \\
\mathbf{P}\left[ W (\widehat{P}_{n}, P) \geq  \rho \right]  \leq \begin{cases}c_{1} \exp \left(-c_{2} n \rho^{\max \{d+1,2\}}\right) & \text { if } \rho \leq 1 \\ c_{1} \exp \left(-c_{2} n \rho^{a}\right) & \text { if } \rho>1\end{cases}
$$
where $c_{1}, c_{2}$ are constants depending on $a, A$ and $d$.
\end{proposition}
As a consequence of this proposition,  for any $\delta > 0$, we have  
\begin{align}\label{E:deltarho}
\mathbf{P}\left[ W (\widehat{P}_{n}, P) \leq  \widehat{\rho}_{n}^{\delta} \right] \geq 1 - \delta \; \text{  where  } \; \widehat{\rho}_{n}^{\delta} \defeq \begin{cases}\left(\frac{\log \left(c_{1} / \delta \right)}{c_{2} n}\right)^{\min \{1 / (d+1), 1 / 2\}} & \text { if } n \geq \frac{\log \left(c_{1} / \delta\right)}{c_{2}}, \\ \left(\frac{\log \left(c_{1} / \delta\right)}{c_{2} n}\right)^{1 / \alpha} & \text { if } n<\frac{\log \left(c_{1} / \delta\right)}{c_{2}}.\end{cases}
\end{align}

\begin{corollary}
	With all assumptions as in Theorem~, we have
	\[ 
	\mathscr{L}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}})- \inf_{f \in \mathcal{F}} \mathscr{L}(P_{\lambda}, f) \leq  \sum_{i=1}^{m} \lambda_i \BiggS{\frac{48 \mathscr{C}(\Theta)}{\sqrt{n_i}} + 2 M_{\ell} \sqrt{\frac{2 \log (4  m / \delta)}{n_i}} + \bigP{2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}} }\widehat{\rho}_{n_i}^{\delta/2m} } +\varepsilon
	\]
	with probability at least $1 - \delta$. 
\end{corollary}
\begin{proof}
We will exploit the joint convexity property of 1-Wasserstein distance, which can be shown as the mapping $(\alpha, \beta) \mapsto W(\alpha, \beta)$ is convex. To see that, by Kantorovich-Rubinstein Duality,  we have $W(\alpha, \beta) = \sup_{\norm{f}_L \leq 1} \mathbf{E}_{\alpha}[f] - \mathbf{E}_{\beta}[f] =  \sup_{\norm{f}_L \leq 1} T_f (\alpha, \beta)$, which is the sumpremum of linear functions $T_f: \gP \times \gP \mapsto \mathbb{R}$ defined by $T_f (\alpha, \beta) = (\alpha, \beta)^{\top}(f, -f)$, and thus the convexity follows. Thus we have 
\begin{align}
W(P_{\lambda}, \widehat{P}_{\lambda}) = W \BigP{\sum\limits_{i=1}^m \lambda_i (\widehat{P}_i, P_i)} \leq  {\sum\limits_{i=1}^m \lambda_i W(\widehat{P}_i, P_i)}.
\end{align}
Then, we have
\begin{align}
\mathbf{P}\BigS{W(P_{\lambda}, \widehat{P}_{\lambda}) \geq \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m} }
&\leq \mathbf{P}\BigS{\sum\limits_{i=1}^m \lambda_i W(\widehat{P}_i, P_i) \geq \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m} } \nonumber\\
&\leq \sum\limits_{i=1}^m  \mathbf{P}\BigS{ W(\widehat{P}_i, P_i) \geq   \widehat{\rho}_{n_i}^{\delta/2m} } \nonumber\\
&\leq \sum\limits_{i=1}^m  \frac{\delta}{2 m}= \frac{\delta}{2}, \label{E:barry}
\end{align}
where the second inequality is due to the union bound, and the third inequality is due to  Proposition~\ref{WassRate} and \eqref{E:deltarho}. By setting $\rho = \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m}$  in Theorem~\ref{Thrm:key} and using union bound, we complete the proof. 
\end{proof}

\subsection{How to choose $\lambda$}
Controlling $\lambda$ for various purpose: either adapt to a specific domain or covering all clients with minimum $\rho$. 

For domain adaptation
\begin{align}
\min_{\lambda \in \Delta} W(\widehat{P}_{\lambda}, \widehat{Q}) \leq \min_{\lambda \in \Delta} \sum\limits_{i=1}^{m} \lambda_i W(\widehat{P}_i, \widehat{Q}) 
\end{align}

For covering all client distribution, based on the Wasserstein barycenter problem
\begin{align}
W(\widehat{P}_{{\lambda}^*}, {P}^*) \leq  \min_{\lambda \in \Delta, Q \in \gP} \sum\limits_{i=1}^{m} \lambda_i W(\widehat{P}_i, {Q}) \defeq \rho^*
\end{align}

By triangle inequality:
\begin{align}
W(P_{\lambda^*}, P_j) &\leq W(P_{\lambda^*}, \widehat{P}_{\lambda^*}) + W(\widehat{P}_{\lambda^*}, P^*) + W( P^*, \widehat{P}_j) + W(  \widehat{P}_j, P_j) \nonumber\\
& \leq \sum\limits_{i=1}^{m} \lambda_i^* \widehat{\rho}_{n_i}^{\delta/2m} + \rho^* + \frac{\rho^*}{\lambda_j} + \widehat{\rho}_{n_j}^{\delta/2} \; \text{  with probability at least }  1-\delta, \label{E:bary2}
\end{align}
where \eqref{E:bary2} is due to several facts: (i) $\mathbf{P}\bigS{W(P_{\lambda^*}, \widehat{P}_{\lambda^*}) \geq \sum\limits_{i=1}^{m} \lambda_i^* \widehat{\rho}_{n_i}^{\delta/2m} } \leq \delta/2$ according to \eqref{E:barry}, (ii) $W( P^*, \widehat{P}_j) = \frac{\lambda_j W( P^*, \widehat{P}_j)}{\lambda_j}\leq \frac{\rho^*}{\lambda_j}$, and (iii)  $\mathbf{P}\bigS{W(  \widehat{P}_j, P_j) \geq \widehat{\rho}_{n_j}^{\delta/2} } \leq \delta/2$ according to \eqref{E:deltarho}, and (iv) using union bound. 

\begin{lemma}
\begin{align*}
	\mathscr{L}_{\rho}^{\gamma}(Q, f) & = \mathscr{L}_{\rho}^{\gamma}(Q,f) + \mathscr{L}_{\rho_{\gamma}}^{\gamma}(Q,f) - \mathscr{L}_{\rho}^{\gamma}(Q,f) \\		
	& = \mathscr{L}_{\rho}^{\gamma}(Q, f)+\gamma(\rho - f_{\gamma}) \\
	& \leq  \mathscr{L}(Q, f) + (2L + \gamma\mathbf{I}_{\{\gamma \neq \gamma^{\prime}\}})\rho		
\end{align*}
\end{lemma}

\textbf{Tuning}:
\begin{enumerate}
	\item Choose the desire $\rho^{*}$
	\item Adjust $\gamma$ to have $\rho_{\gamma} = \rho^{*}$
\end{enumerate}


